Think Eternally: Improved Algorithms for the Temp Secretary Problem and Extensions

The \emph{Temp Secretary Problem} was recently introduced by Fiat et al. It is a generalization of the Secretary Problem, in which commitments are temporary for a fixed duration. We present a simple online algorithm with improved performance guarantees for cases already considered by Fiat et al.\ and give competitive ratios for new generalizations of the problem. In the classical setting, where candidates have identical contract durations $\gamma \ll 1$ and we are allowed to hire up to $B$ candidates simultaneously, our algorithm is $(\frac{1}{2} - O(\sqrt{\gamma}))$-competitive. For large $B$, the bound improves to $1 - O\left(\frac{1}{\sqrt{B}}\right) - O(\sqrt{\gamma})$. Furthermore we generalize the problem from cardinality constraints towards general packing constraints. We achieve a competitive ratio of $1 - O\left(\sqrt{\frac{(1+\log d + \log B)}{B}}\right) -O(\sqrt{\gamma})$, where $d$ is the sparsity of the constraint matrix and $B$ is generalized to the capacity ratio of linear constraints. Additionally we extend the problem towards arbitrary hiring durations. Our algorithmic approach is a relaxation that aggregates all temporal constraints into a non-temporal constraint. Then we apply a linear scaling algorithm that, on every arrival, computes a tentative solution on the input that is known up to this point. This tentative solution uses the non-temporal, relaxed constraints scaled down linearly by the amount of time that has already passed.

==> different_lengths_largeb.tex <==
\begin{theorem}\label{theorem:different_length_simultaneous}
The linear scaling algorithm is $\left(1 - \Theta\left(\sqrt{\frac{\log B}{B}}\right) - \Theta(\sqrt{\gamma})\right)$-competitive for the temp secretary problem with arbitrary contract length $\lambda_j\leq \gamma$.
\end{theorem}

\begin{proof}[Proof (of Theorem~\ref{theorem:different_length_simultaneous})]
Let $X_{i, \ell-i}$ be a random variable that is $1$ if the event $H_{i, \ell-i}$ occurs and $0$ otherwise. Then the probability that a tentative hire in round $\ell$ is feasible is

\[\Pr{\mbox{hire in }\ell\mbox{ feasible}} \geq 1 - \Pr{\sum_{i=1}^{\gamma N} X_{i, \ell-i} \geq B}\]

From Lemma~\ref{lemma:tentative_length} we have

\[\Ex{\sum_{i=1}^{\gamma N} X_{i, \ell-i}} \leq \sum_{i=1}^{\gamma N} \left(\Ex{X_{i, \ell}} + \frac{B}{\ell - i}\right)\enspace.\]

The sum $\sum_{i=1}^{\gamma N} \Ex{X_{i, \ell}}$ is exactly the expected length of a tentative hire made in round $\ell$. Since the capacity in round $\ell$ is $\alpha B \ell$ the expected capacity used by the candidate arriving in round $\ell$ is $\alpha B$. We have $\frac{B}{\ell-i}\leq \frac{B}{\ell - \gamma N}$ for all relevant $i$ and with $\alpha = 1 - 2\epsilon$ and $\epsilon = 2\sqrt{\gamma} + \sqrt{\frac{\log B}{B}}$ we have for all $\ell > \sqrt{\gamma} N$

\begin{align*}
\Ex{\sum_{i=1}^{\gamma N} X_{i, \ell-i}} &\leq (1 - 2\epsilon) B + \frac{\gamma N B}{\ell - \gamma N}\\
&\leq\left(1-\epsilon-2\sqrt{\gamma} - \sqrt{\frac{\log B}{B}}+\frac{\gamma}{\sqrt{\gamma} - \gamma}\right) B\leq (1-\epsilon)B\enspace.
\end{align*}

Now we use a Chernoff bound with $\delta = 1 - 3\sqrt{\frac{\log B}{b}}$ and get \todo{why can we do this?}

\begin{align*}
\Pr{\mbox{hire in }\ell\mbox{ feasible}} &\geq 1 - \Pr{\sum_{i=1}^{\gamma N} X_{i, \ell-i} \geq (1+\delta)(1-\epsilon)B}\\
&\geq 1 - e^{-\frac{\delta^2(1-\epsilon)B}{3}} = 1 - e^{-3\log B (1-\epsilon)} \geq 1 - \frac{1}{B} \enspace.
\end{align*}

In combination with Lemma~\ref{lemma:STOC} we now compute the expected value collected by the algorithm

\begin{align*}
\Ex{\sum_{i \in \ALG} v_i} &\geq \sum_{i=2}^{\frac{1}{\sqrt{\gamma}}-1} \sum_{\ell=i\sqrt{\gamma}N}^{(i+1)\sqrt{\gamma}N-1}\frac{\Ex{v\left(S^{(\ell)}\right)}}{\ell}\cdot \Pr{\mbox{hire in }\ell\mbox{ feasible}}\\
&\geq \sum_{i=2}^{\frac{1}{\sqrt{\gamma}}-1} \sum_{\ell=i\sqrt{\gamma}N}^{(i+1)\sqrt{\gamma}N-1}\alpha\cdot\frac{\left(1 - 9 \sqrt{\frac{\gamma}{\nicefrac{\ell}{N}}} \right)\frac{\ell}{N}\Ex{\sum_{i \in \OPT} v_i}}{\ell}\left(1-\frac{1}{B}\right)\enspace.
\end{align*}

First we bound the inner sum with the smallest term. Then we do all the multiplications and ignore the positive terms.

\begin{align*}
\Ex{\sum_{i \in \ALG} v_i} &\geq \sum_{i=2}^{\frac{1}{\sqrt{\gamma}}-1}\sqrt{\gamma}N \left(1 - 2\sqrt{\gamma} - \sqrt{\frac{\log B}{B}}\right) \left(1 - 9 \sqrt{\frac{\gamma}{i\sqrt{\gamma}}}\right)\frac{\Ex{\sum_{i \in \OPT} v_i}}{N}\cdot\left(1-\frac{1}{B}\right)\\
&\geq \sqrt{\gamma} \sum_{i=2}^{\frac{1}{\sqrt{\gamma}}-1} \left(1 - 2\sqrt{\gamma} - \sqrt{\frac{\log B}{B}} - \frac{1}{B} - 9 \sqrt{\frac{\gamma}{i\sqrt{\gamma}}} \right)\Ex{\sum_{i \in \OPT} v_i}\enspace.
\end{align*}

Finally we solve the last remaining sum. Again we use the integral $\int \frac{1}{\sqrt{x}}dx = 2\sqrt{x}$ and ignore all inessential, positive terms.

\begin{align*}
\Ex{\sum_{i \in \ALG} v_i}&\geq\left(1-2\sqrt{\gamma}\right)\cdot\left(1 - 2\sqrt{\gamma} - \sqrt{\frac{\log B}{B}} - \frac{1}{B} - 18 \sqrt{\gamma} \right)\Ex{\sum_{i \in \OPT} v_i}\\
&\geq \left(1 - 22\sqrt{\gamma} - \sqrt{\frac{1 + \log B}{B}}\right)\Ex{\sum_{i \in \OPT} v_i}\enspace.
\end{align*}
\end{proof}


==> model.tex <==



\subsection{Model}

We consider the temp secretary problem arbitrary distribution of arrival times. In this problem an adversary generates candidates $j\in U$ with value $v_j$ and contract length $\alpha_j$. Then a random arrival time $\theta(j) \sim F[0,1]$ is assigned to every candidate.

Furthermore we bound $\alpha_j$ by $\gamma \geq F(\theta(j) + \alpha_j) - F(\theta(j))$. Therefore, if $F$ is the uniform distribution $\gamma$ is the maximal length of a contract $\alpha_j \leq \gamma$ for all contracts $j$.

On every arrival the online algorithm has to make an irrevocable decision whether to hire the candidate or not. Additionally, there might be constraints on the candidates that can be hired simultaneously. In the most simple case in Section~\ref{sec:temp_basic} only a single candidate can be hired at a time and the next one can only be hired after the first contract has expired. In Section~\ref{sec:temp_packing} we allow packing constraints that correspond to a packing linear program for all active contracts for all $t\in[0, 1]: \sum_{j: \theta(j) > t - \alpha_j} a_{i, j} x_j \leq b_i$. Intuitively the constraints are over types of candidates hired at a time. Every candidate can have several types to different fractional degrees. \todo{translate: Ausprägungen}
